Search for an additional, heavy Higgs boson in the $H\rightarrow ZZ$ decay channel at $\sqrt{s}$ = 8 TeV in $pp$ collision data with the ATLAS detector

A search is presented for a high-mass Higgs boson in the $H\rightarrow\ell\ell\ell\ell$, $H\rightarrow\ell\ell\nu\nu$, $H\rightarrow\ell\ell qq$, and $H\rightarrow\nu\nu qq$ decay modes using the ATLAS detector at the CERN Large Hadron Collider. The search uses proton-proton collision data at a centre-of-mass energy of 8 TeV corresponding to an integrated luminosity of 20.3 fb$^{-1}$. The results of the search are interpreted in the scenario of a heavy Higgs boson with a width that is small compared with the experimental mass resolution. The Higgs boson mass range considered extends up to 1 TeV for all four decay modes and down to as low as 140 GeV, depending on the decay mode. No significant excess of events over the Standard Model prediction is found. A simultaneous fit to the four decay modes yields upper limits on the production cross-section of a heavy Higgs boson times the branching ratio to Z boson pairs. 95% confidence level upper limits range from 0.53 pb at $m_H=195$ GeV to 0.008 pb at $m_H=950$ GeV for the gluon-fusion production mode and from 0.31 pb at $m_H=195$ GeV to 0.009 pb at $m_H=950$ GeV for the vector-boson-fusion production mode. The results are also interpreted in the context of Type-I and Type-II two-Higgs-doublet models.

==> atlas-document-metadata.tex <==
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used by the different cover pages.
%-------------------------------------------------------------------------------

% Title
\AtlasTitle{Search for an additional, heavy Higgs boson in the \htozz\ decay channel at $\sqrt{s} = 8\;\mbox{TeV}$ in $pp$ collision data with the ATLAS detector}

% Author - this does not work with revtex (add it after \begin{document})
\author{The ATLAS Collaboration}

% Authors and list of contributors to the analysis
% \AtlasAuthorContribute also adds the name to the author list
% Include package latex/atlascontribute to use this
% Use authblk package if there are multiple authors, which is included by latex/atlascontribute
% \usepackage{authblk}
% \renewcommand\Authands{, } % avoid ``. and'' for last author
% \renewcommand\Affilfont{\itshape\small} % affiliation formatting
% \AtlasAuthorContributor{First AtlasAuthorContributor}{a}{Author's contribution.}
% \AtlasAuthorContributor{Second AtlasAuthorContributor}{b}{Author's contribution.}
% \AtlasAuthorContributor{Third AtlasAuthorContributor}{a}{Author's contribution.}
% \AtlasContributor{Fourth AtlasContributor}{Contribution to the analysis.}
% \author[a]{First Author}
% \author[a]{Second Author}
% \author[b]{Third Author}
% \affil[a]{One Institution}
% \affil[b]{Another Institution}

% If a special author list should be indicated via a link use the following code:
% Include the two lines below if you do not use atlasstyle:
% \usepackage[marginal,hang]{footmisc}
% \setlength{\footnotemargin}{0.5em}
% Use the following lines in all cases:
% \usepackage{authblk}
% \author{The ATLAS Collaboration%
% \thanks{The full author list can be found at:\newline
%   \url{https://atlas.web.cern.ch/Atlas/PUBNOTES/ATL-PHYS-PUB-2014-007/authorlist.pdf}}
% }

% Date: if not given, uses current date
%\date{\today}

% Draft version:
% Should be 1.0 for the first circulation, and 2.0 for the second circulation.
% If given, adds draft version on front page, a 'DRAFT' box on top of each other page, 
% and line numbers.
% Comment or remove in final version.
\AtlasVersion{3.1}

% ATLAS reference code, to help ATLAS members to locate the paper
\AtlasRefCode{HIGG-2013-20}

% ATLAS note number. Can be an COM, INT, PUB or CONF note
% \AtlasNote{ATLAS-CONF-2014-XXX}
% \AtlasNote{ATL-PHYS-PUB-2014-XXX}
% \AtlasNote{ATL-COM-PHYS-2014-XXX}

% CERN preprint number
\PreprintIdNumber{CERN-PH-EP-2015-154}

% ATLAS date - arXiv submission; to be filled in by the Physics Office
% \AtlasDate{\today}

% arXiv identifier
% \arXivId{14XX.YYYY}

% HepData record
% \HepDataRecord{ZZZZZZZZ}

% Submission journal and final reference
% \AtlasJournal{Phys.\ Lett.\ B.}
% \AtlasJournalRef{\PLB 789 (2014) 123}
% \AtlasDOI{}
\AtlasJournal{EPJC}

% Abstract - % directly after { is important for correct indentation
\AtlasAbstract{%
  A search is presented for a high-mass Higgs boson in the \htollll, \htollvv, \htollqq, and \htovvqq\  
  decay modes using the ATLAS detector at the CERN
  Large Hadron Collider. The search uses proton--proton collision data at a
  centre-of-mass energy of 8~TeV corresponding to an integrated luminosity of 20.3~fb$^{-1}$. The
  results of the search are interpreted in the scenario of a heavy Higgs boson
  with a width that is small compared with the experimental mass resolution.
  The Higgs boson mass range considered extends up to $1\tev$ for all four decay modes and down to as low as $140\gev$, depending on the decay mode.
No significant excess of events over the Standard Model prediction is found.
A simultaneous fit to the four decay modes yields upper limits on the production
cross-section of a heavy Higgs~boson times the branching ratio
to $Z$~boson pairs.  
%95\% confidence level upper limits
  %range from 0.19~pb (at $m_H=140\gev$) to 0.011~pb (at $m_H=1\tev$) for the gluon-fusion
  %production
  %mode, and from 0.20~pb (at $m_H=140\gev$) to
  %0.013~pb at ($m_H=1\tev$) for the vector-boson-fusion production mode. 
  95\% confidence level upper limits
  range from 0.53~pb at $\mH=195$~\gev\ to 0.008~pb at $\mH=950$~\gev\ for the
  gluon-fusion production mode and
  from 0.31~pb at $\mH=195$~\gev\ to 0.009~pb at $\mH=950$~\gev\ 
  for the vector-boson-fusion production mode.
  The results are also interpreted in the context
  of Type-I and Type-II two-Higgs-doublet models.
}

%-------------------------------------------------------------------------------
% The following information is needed for the cover page. The commands are only defined
% if you use the coverpage option in atlasdoc or use the atlascover package
%-------------------------------------------------------------------------------

% List of supporting notes  (leave as null \AtlasCoverSupportingNote{} if you want to skip this option)
% \AtlasCoverSupportingNote{Short title note 1}{https://cds.cern.ch/record/XXXXXXX}
% \AtlasCoverSupportingNote{Short title note 2}{https://cds.cern.ch/record/YYYYYYY}
\AtlasCoverSupportingNote{\htollqq}{https://cds.cern.ch/record/1693159}
\AtlasCoverSupportingNote{\htollvv}{https://cds.cern.ch/record/1693161}
\AtlasCoverSupportingNote{\htollll}{https://cds.cern.ch/record/1693487}
\AtlasCoverSupportingNote{\htovvqq}{https://cds.cern.ch/record/1692942}
%\AtlasCoverSupportingNote{Model Interpretation}{https://cds.cern.ch/record/1692903}
\AtlasCoverSupportingNote{Combination}{https://cds.cern.ch/record/1995509}
%
% OR (the 2nd option is deprecated, especially for CONF and PUB notes)
%
% Supporting material TWiki page  (leave as null \AtlasCoverTwikiURL{} if you want to skip this option)
% \AtlasCoverTwikiURL{https://twiki.cern.ch/twiki/bin/view/Atlas/WebHome}

% Comment deadline
\AtlasCoverCommentsDeadline{25 June 2015}

% Analysis team members - contact editors should no longer be specified
% as there is a generic email list name for the editors
% \AtlasCoverAnalysisTeam{Peter Analyser, Susan Editor1, Jenny Editor2, Alphonse Physicien}
\AtlasCoverAnalysisTeam{
S.~H.~Abidi,
C.~Anastopoulos,
S.~Angelidakis,
L.~Aperio Bella,
G.~Artoni,
M.~Baak,
P.~Clark,
F.~Conventi,
R.~Di~Nardo,
T.~Donszelmann Cuhadar,
N.~Edwards,
D.~Fassouliotis,
G.~Garrillo Montoya,
F.~Garay Walls,
C.~Gwilliam,
M.~Hoffmann,
R.~Harrington,
X.~Ju,
L.S.~Kaplan,
D.~Kyriazopoulos,
A.~Mehta,
E.~Mountricha,
R.~Nicolaidou,
S.~Oda,
H.~Okawa,
K.~Parker,
A.~Sanchez Pineda,
J.~Price,
M.~Rescigno,
C.~Savarese,
F.~Lo Sterzo,
S.~Snyder,
J.~Voosebeld,
C.~Wang,
S.M.~Wang,
S.L.~Wu,
L.~Xu,
L.~Zhang,
Z.~Zhao,
B.~Zhou,
G.~Zurzolo
}

% Editorial Board Members - indicate the Chair by a (chair) after his/her name
% Give either all members at once (then they appear on one line), or separately
% \AtlasCoverEdBoardMember{EdBoard~Chair~(chair), EB~Member~1, EB~Member~2, EB~Member~3}
% \AtlasCoverEdBoardMember{EdBoard~Chair~(chair)}
% \AtlasCoverEdBoardMember{EB~Member~1}
% \AtlasCoverEdBoardMember{EB~Member~2}
% \AtlasCoverEdBoardMember{EB~Member~3}
\AtlasCoverEdBoardMember{M.~Vos~(chair)}
\AtlasCoverEdBoardMember{V.~Cavaliere}
\AtlasCoverEdBoardMember{P.~Maettig}
\AtlasCoverEdBoardMember{D.~Whiteson}

% A PUB note has readers and not an EdBoard -- give their names here (one line or several entries)
% \AtlasCoverReaderMember{Reader~1, Reader~2}
% \AtlasCoverReaderMember{Reader~1}
% \AtlasCoverEdBoardMember{Reader~2}

% Editors egroup
% \AtlasCoverEgroupEditors{atlas-GROUP-2014-XX-editors@cern.ch}
\AtlasCoverEgroupEditors{atlas-HIGG-2013-20-editors@cern.ch}

% EdBoard egroup
% \AtlasCoverEgroupEdBoard{atlas-GROUP-2014-XX-editorial-board@cern.ch}
\AtlasCoverEgroupEdBoard{atlas-HIGG-2013-20-editorial-board@cern.ch}


